A Fleet of Miniature Cars for Experiments in Cooperative Driving

We introduce a unique experimental testbed that consists of a fleet of 16 miniature Ackermann-steering vehicles. We are motivated by a lack of available low-cost platforms to support research and education in multi-car navigation and trajectory planning. This article elaborates the design of our miniature robotic car, the Cambridge Minicar, as well as the fleet's control architecture. Our experimental testbed allows us to implement state-of-the-art driver models as well as autonomous control strategies, and test their validity in a real, physical multi-lane setup. Through experiments on our miniature highway, we are able to tangibly demonstrate the benefits of cooperative driving on multi-lane road topographies. Our setup paves the way for indoor large-fleet experimental research.

==> sec_software.tex <==
%---------------------------------------------------------
\section{Open-Source Tools}
\label{sec:software}

Our design and the software tools are available in a GitHub repository ({\footnotesize{\url{https://github.com/proroklab/minicar}}}).

% calibration procedure.
% player code
% car (listener) code.
% We also provide the design guidelines, bill-of-materials.}

